On Some Applications of Group Representation Theory to Algebraic Problems Related to the Congruence Principle for Equivariant Maps

Given a finite group $G$ and two unitary $G$-representations $V$ and $W$, possible restrictions on Brouwer degrees of equivariant maps between representation spheres $S(V)$ and $S(W)$ are usually expressed in a form of congruences modulo the greatest common divisor of lengths of orbits in $S(V)$ (denoted $\alpha(V)$). Effective applications of these congruences is limited by answers to the following questions: (i) under which conditions, is ${\alpha}(V)>1$? and (ii) does there exist an equivariant map with the degree easy to calculate? In the present paper, we address both questions. We show that ${\alpha}(V)>1$ for each irreducible non-trivial $C[G]$-module if and only if $G$ is solvable. For non-solvable groups, we use 2-transitive actions to construct complex representations with non-trivial ${\alpha}$-characteristic. Regarding the second question, we suggest a class of Norton algebras without 2-nilpotents giving rise to equivariant quadratic maps, which admit an explicit formula for the Brouwer degree.

==> g32_irr_lat_orbtypes.tex <==
  \begin{figure}[h]
    \centering
    \subfigure[$\rho_1$]{
    \includegraphics[scale=.3]{g_lat_irr_stab4}}\quad
    \subfigure[$\rho_2$]{
    \includegraphics[scale=.3]{g_lat_irr_stab5}}\quad
    \subfigure[$\rho_3$]{
    \includegraphics[scale=.3]{g_lat_irr_stab6}}\quad
    \subfigure[$\rho_4$]{
    \includegraphics[scale=.3]{g_lat_irr_stab7}}
    \caption{lattice of orbit types of
        $\rho\in\varrho^a(V\rtimes\gl(3,2))$}
    \label{fig:g_irr_lat_orbtypes}
  \end{figure}


==> s5_irr_lat_orbtypes.tex <==
  \begin{figure}[h]
    \centering
    \subfigure[$\rho_1$]{
    \includegraphics[scale=.3]{s5_lat_irr_stab1}}\quad
    \subfigure[$\rho_3$]{
    \includegraphics[scale=.3]{s5_lat_irr_stab3}}\quad
    \subfigure[$\rho_6$]{
    \includegraphics[scale=.3]{s5_lat_irr_stab6}}
    \caption{lattice of orbit types of
        $\rho\in\varrho^a(S_5))$}
    \label{fig:s5_irr_lat_orbtypes}
  \end{figure}

